Component-aware Orchestration of Cloud-based Enterprise Applications, from TOSCA to Docker and Kubernetes

Enterprise IT is currently facing the challenge of coordinating the management of complex, multi-component applications across heterogeneous cloud platforms. Containers and container orchestrators provide a valuable solution to deploy multi-component applications over cloud platforms, by coupling the lifecycle of each application component to that of its hosting container. We hereby propose a solution for going beyond such a coupling, based on the OASIS standard TOSCA and on Docker. We indeed propose a novel approach for deploying multi-component applications on top of existing container orchestrators, which allows to manage each component independently from the container used to run it. We also present prototype tools implementing our approach, and we show how we effectively exploited them to carry out a concrete case study.

==> src/old/3-big-picture.tex <==
Our ultimate objective is to enable a component-aware management of multi-component applications by piggybacking on existing container orchestrators (such as Docker Swarm and Kubernetes). 
We indeed aim at seamlessly extending the support they provide for orchestrating containers, so that the lifecycle of application components is not entangled to that of their hosting containers, but rather allowing components to be managed independently.

Fig.~\ref{fig:big-picture} provides an high-level overview on the orchestration approach we propose.
Starting from the CSAR archive containing the specification of a multi-component application and of its container-based deployment, a \textit{translator} generates a new artifact (based on Docker Compose), which allows deploying the application on top of Docker-compliant container orchestrators.
The obtained artifact not only packages the components forming an application within the containers hosting them, but also seamlessly extends the application deployment by introducing some additional components enabling the desired component-aware orchestration.
\begin{itemize}
	\item A \textit{worker} (\textit{w} in the figure) is included in each container packaging some application components. 
	The worker is responsible of managing the lifecycle of the components packaged within the container it appears in, by launching the concrete artifacts (\eg bash scripts) implementing their management operations.
	\item A \textit{manager} (\textit{m} in the figure) is included and packaged within a separate container.
	The manager is responsible of interacting and coordinating the workers, in order to manage the components forming an application, and based on the commands issued by an application administrator.
\end{itemize}

\begin{figure}
  \centering
  \includegraphics[scale=\figscale]{fig/big-picture}
  \caption{Bird-eye view of our approach for enabling a component-aware orchestration of the management multi-component applications on top of existing container orchestrators.}
  \label{fig:big-picture}
\end{figure}

With our approach, an application administrator can continue to deploy and manage the containers in an application by exploiting existing container orchestrators.
She can then deploy and manage each software component forming her application by issuing commands to the containerised manager, which will then properly forward it to the workers to enact the corresponding management operation.
\comment{Matteo}{L'utilizzo del femminile \`e una forma di cortesia.}
For instance, once the containers in Fig.~\ref{fig:big-picture} are all running, an application administrator may issue the commands to install and start service \textit{s1} to the manager.
The latter will forward the corresponding requests to the worker in the container \textit{c1}, which will launch the bash scripts implementing the to-be-enacted management operations.

It is worth noting that our approach seamlessly integrates with any Docker-compliant container orchestrator, as the newly introduced components (\ie the manager and the workers) are themselves packaged within Docker containers.
In addition, by piggybacking on existing container orchestrator, our approach allows to uniformly manage containers, independently on whether they are used as lightweight virtual hosting environments for application components (as \textit{c1} e \textit{c4} in the figure) or whether they are used as standalone services (as \textit{c2} in the figure).
This allows application administrators to choose whether to enable the fine-grain management of components or to couple their lifecycle to the containers they appear in.
In the former case, she has to distinguish components and containers in the TOSCA application specification (and provide the artifacts implementing the lifecycle operations of such components), while in the latter case she just packages the components within the corresponding containers (by writing proper Dockerfiles --- as she would be doing with current Docker-based orchestrators).

\smallskip \noindent
In the following, we illustrate how we concretely obtained the above illustrated orchestration solution, by designing and developing the \toskose open-source \rev{toolset}. 
We first show the issues and design choices for allowing \textit{workers} to independently manage the software components packaged within a container (Sect.~\ref{sec:toskose-unit}).
We then show how we concretised the \textit{manager} to enable the orchestration of multi-component applications on top of existing orchestrator (Sect.~\ref{sec:toskose-manager}), and how we implemented the \textit{translator} for generating a Docker-based artifacts from the TOSCA specification of an application (Sect.~\ref{sec:packaging}). 


